Deep Denoising Prior-Based Spectral Estimation for Phaseless Synthetic Aperture Radar

Incoherent processing for synthetic aperture radar (SAR) is a promising approach that enables low implementation costs, simplified hardware designs and operations in high frequency spectrum compared to the conventional imaging methods using coherent processing. Existing non-convex phaseless imaging algorithms offer recovery guarantees over limited range of forward models. In recent years, several deep learning (DL) based techniques have been introduced with the goal of extending applicability of phaseless imaging techniques to wave-based imaging modalities by addressing fundamental challenges, such as, lack of redundancy, non-uniqueness issues encountered commonly with inverse scattering models. In this paper, we introduce a DL-based phaseless SAR imaging approach that is designed under the premise that the spectral estimation technique, widely used for initializing non-convex phase retrieval algorithms, has significance far beyond generating good initial points. We extend the iterative power method for spectral estimation by using deep denoisers at each iteration, and subsequently design a deep imaging network within the plug-and-play framework. Finally, we verify the feasibility of our approach using synthetic SAR measurements.

==> back_up.tex <==
In this section, we verified the feasibility of our approach by using simulated SAR scenes and corresponding intensity measurements.
We considered two datasets, one with a single extended and randomly located rectangular target of random dimensions in the scene; the second consists of randomly located and random number of point target within the area being imaged.
For both cases, training datasets have $5000$ samples, each having the ground truth image and the corresponding SAR intensity measurements available, while the test datasets contain $50$ samples with only the intensity measurements for each sample.
For both datasets, the area within the SAR field of view is assumed to have an area of $62$ m $\times 62$ m.
Central frequency and transmission bandwidth are $9.9$ GHz and $75$ MHz, respectively.
We assume spot-light mode SAR with a circular trajectory with radius $10$ km, aperture length $\pi$ radian and an altitude of $7$ km.
We reconstruct the scenes from the extended and point targets datasets, respectively, as $31 \times 31$ and $40 \times 40$ pixels image vectors.
For both cases, the $M/N$ ratios are $2$ with the number of slow time point, distributed over the aperture at equi-distant points, equal to $62$ for the extended target data and $80$ for the dataset with point target.
Moreover, for both cases, we consider the presence of additive Gaussian distributed noise of $10$ dB on the measured intensity values of the scattered signals.

We implement the denoiser using convolution neural networks (CNN) with $16$ convolution layers and
We implemented our unrolled imaging network from Fig.~\ref{fig:network_model_phaseless_SAR} by using $4$ and $8$ iterations, respectively, for the reconstructing the rectangular and point target images.
Also, to limit the total number of trainable parameter, we gradually increased these numbers and used the same denoiser for all two consecutive layers.
Two example reconstructed images are shown in Fig.~\ref{}, along with corresponding ground truth images and the reconstructed images using the WF algorithm~\cite{candes2015phase_IEEE, yonel2020deterministic}.



At the low $M/N$ ratios used in these reconstructions, our approach out-performs the WF algorithm in terms of mean squared error (MSE) metric.
Average computation times for our approach and the WF algorithms required to attain these MSE values are   and     , respectively, indicating an improvement in computation time by our approach.







